Efficient recovery-based error estimation for the smoothed finite element method for smooth and singular linear elasticity

An error control technique aimed to assess the quality of smoothed finite element approximations is presented in this paper. Finite element techniques based on strain smoothing appeared in 2007 were shown to provide significant advantages compared to conventional finite element approximations. In particular, a widely cited strength of such methods is improved accuracy for the same computational cost. Yet, few attempts have been made to directly assess the quality of the results obtained during the simulation by evaluating an estimate of the discretization error. Here we propose a recovery type error estimator based on an enhanced recovery technique. The salient features of the recovery are: enforcement of local equilibrium and, for singular problems a "smooth+singular" decomposition of the recovered stress. We evaluate the proposed estimator on a number of test cases from linear elastic structural mechanics and obtain precise error estimations whose effectivities, both at local and global levels, are improved compared to recovery procedures not implementing these features.

==> babelbst.tex <==
%%
%% This is file `esbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% spanish.dtx  (with options: `bblbst')
%% This is a generated file.
%% 
%% Copyright 1989-2005 Johannes L. Braams and any individual authors
%% listed elsewhere in this file.  All rights reserved.
%% 
%% This file was generated from file(s) of the Babel system.
%% ---------------------------------------------------------
%% 
%% It may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%% 
%% This work has the LPPL maintenance status "maintained".
%% 
%% The Current Maintainer of this work is Johannes Braams.
%% 
%% This file may only be distributed together with a copy of the Babel
%% system. You may however distribute the Babel system without
%% such generated files.
%% 
%% The list of all files belonging to the Babel distribution is
%% given in the file `manifest.bbl'. See also `legal.bbl for additional
%% information.
%% 
%% The list of derived (unpacked) files belonging to the distribution
%% and covered by LPPL is defined by the unpacking scripts (with
%% extension .ins) which are part of the distribution.
%% File `spanish.dtx'
%% Babel package for LaTeX version 2e
%% Copyright (C) 1989 - 2004
%%           by Johannes Braams, TeXniek
%% Spanish Language Definition File
%% Copyright (C) 1997 - 2005
%%           by Javier Bezos (jbezos at wanadoo.es)
%%           Apartado 116.035
%%           E-28080 Madrid
%%           Espa\~na / Espagne
%%      and
%%           by CervanTeX (www.cervantex.org)
%% Please report errors to: Javier Bezos (preferably)
%%                          jbezos at wanadoo.es
%%                          J.L. Braams
%%                          babel at braams.cistron.nl
%% \section{\textsf{spanish} como lengua principal}
\def\bbland{y}
\def\bbleditors{directores}     \def\bbleds{eds.\@}
\def\bbleditor{director}        \def\bbled{ed.\@}
\def\bbledby{dirigido por}
\def\bbledition{edici\'on}      \def\bbledn{ed.\@}
\def\bbletal{y otros}
\def\bblvolume{vol\'umen}       \def\bblvol{vol.\@}
\def\bblof{de}
\def\bblnumber{n\'umero}        \def\bblno{n\sptext{o}}
\def\bblin{en}
\def\bblpages{p\'aginas}        \def\bblpp{p\'ags.\@}
\def\bblpage{p\'gina}           \def\bblp{p\'ag.\@}
\def\bblchapter{cap\'itulo}     \def\bblchap{cap.\@}
\def\bbltechreport{informe t\'ecnico}
\def\bbltechrep{inf.\@ t\'ec.\@}
\def\bblmthesis{proyecto de fin de carrera}
\def\bblphdthesis{tesis doctoral}
\def\bblfirst {primera}         \def\bblfirsto {1\sptext{a}}
\def\bblsecond{segunda}         \def\bblsecondo{2\sptext{a}}
\def\bblthird {tercera}         \def\bblthirdo {3\sptext{a}}
\def\bblfourth{cuarta}          \def\bblfourtho{4\sptext{a}}
\def\bblfifth {quinta}          \def\bblfiftho {5\sptext{a}}
\def\bblth{\sptext{a}}
\let\bblst\bblth   \let\bblnd\bblth   \let\bblrd\bblth
\def\bbljan{enero}  \def\bblfeb{febrero}  \def\bblmar{marzo}
\def\bblapr{abril}  \def\bblmay{mayo}     \def\bbljun{junio}
\def\bbljul{julio}  \def\bblaug{agosto}   \def\bblsep{septiembre}
\def\bbloct{octubre}\def\bblnov{noviembre}\def\bbldec{diciembre}
%%
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%
\endinput
%%
%% End of file `esbst.tex'.

